Complementarity between neutrinoless double beta decay and collider searches for heavy neutrinos in composite-fermion models

Composite-fermion models predict excited quarks and leptons with mass scales which can potentially be observed at high-energy colliders like the LHC; the most recent exclusion limits from the CMS and ATLAS Collaborations corner excited-fermion masses and the compositeness scale to the multi-TeV range. At the same time, hypothetical composite Majorana neutrinos would lead to observable effects in neutrinoless double beta decay ($0\nu \beta \beta$) experiments. In this work, we show that the current composite-neutrino exclusion limit $M_N>4.6$ TeV, as extracted from direct searches at the LHC, can indeed be further improved to $M_N>8.8$ TeV by including the bound on the nuclear transition $^{136}$Xe $\to$ $^{136}$Ba $+2e^-$. Looking ahead, the forthcoming HL-LHC will allow probing a larger portion of the parameter-space, nevertheless, it will still benefit from the complementary limit provided by $0 \nu \beta \beta$ future detectors to explore composite-neutrino masses up to $12.6$ TeV.

==> Makefile <==
# input
MAIN					= main

MAIN_TEX				= ${MAIN}.tex
MAIN_PDF				= ${MAIN}.pdf

BIBLIOGRAPHY		= new_ref.bib

# clean
FILE_CLEAN			= *.aux *.bbl *.blg *.brf *.idx *.ilg *.ind *.log *.out *~ *Notes.bib
FILE_DISTCLEAN		= ${MAIN_PDF} ${OUTPUT_PDF}

.PHONY:	pdf biblio \
			rename \
			distclean clean

pdf:	${MAIN_TEX}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
biblio: ${MAIN_TEX} ${BIBLIOGRAPHY} 
	pdflatex ${MAIN}
	bibtex ${MAIN}
#	makeindex ${MAIN}
	pdflatex ${MAIN}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
view:	${MAIN_PDF}
	evince ${MAIN_PDF}
	
distclean:	clean
	rm -f ${FILE_DISTCLEAN}

clean:
	rm -f ${FILE_CLEAN}

